Mora: Enabling Generalist Video Generation via A Multi-Agent Framework

Text-to-video generation has made significant strides, but replicating the capabilities of advanced systems like OpenAI Sora remains challenging due to their closed-source nature. Existing open-source methods struggle to achieve comparable performance, often hindered by ineffective agent collaboration and inadequate training data quality. In this paper, we introduce Mora, a novel multi-agent framework that leverages existing open-source modules to replicate Sora functionalities. We address these fundamental limitations by proposing three key techniques: (1) multi-agent fine-tuning with a self-modulation factor to enhance inter-agent coordination, (2) a data-free training strategy that uses large models to synthesize training data, and (3) a human-in-the-loop mechanism combined with multimodal large language models for data filtering to ensure high-quality training datasets. Our comprehensive experiments on six video generation tasks demonstrate that Mora achieves performance comparable to Sora on VBench, outperforming existing open-source methods across various tasks. Specifically, in the text-to-video generation task, Mora achieved a Video Quality score of 0.800, surpassing Sora 0.797 and outperforming all other baseline models across six key metrics. Additionally, in the image-to-video generation task, Mora achieved a perfect Dynamic Degree score of 1.00, demonstrating exceptional capability in enhancing motion realism and achieving higher Imaging Quality than Sora. These results highlight the potential of collaborative multi-agent systems and human-in-the-loop mechanisms in advancing text-to-video generation. Our code is available at \url{https://github.com/lichao-sun/Mora}.

==> sections/intro-bk.tex <==
Generative AI technologies have significantly reshaped daily life and industry, with substantial progress particularly notable in visual AI through image generation models like Midjourney~\citep{midjourney}, Stable Diffusion~\citep{rombach2022high}, and DALL-E 3~\citep{betker2023improving}. However, video generation, especially for durations exceeding 10 seconds, has not kept pace. Recent developments such as Pika~\citep{pika} and Gen-2~\citep{Gen-2} have shown potential but are limited to short outputs. A major advancement occurred with OpenAI's launch of Sora in February 2024. This text-to-video model can create videos up to a minute long that closely align with text prompts and excels in a variety of video tasks, including editing and extending footage, offering multi-view perspectives, and adhering closely to user instructions~\citep{openai2024sora}.
Despite these innovations, the closed-source nature of Sora presents significant barriers to academic research and development. Attempts to reverse-engineer Sora are exploring potential techniques like diffusion transformers and spatial patch strategies~\citep{sohl2015deep,ho2020denoising,bao2023all,peebles2023scalable}, but the challenge of matching its performance with limited resources remains formidable.


In parallel, autonomous agents employing Large Language Models (LLMs) show promise in replicating and enhancing human workflows. Although existing systems primarily focus on text-based tasks, utilizing well-defined Standard Operating Procedures (SOPs) for task decomposition and agent coordination. SOPs dictate agent responsibilities and set standards for outputs, as seen in platforms like MetaGPT~\citep{hong2023metagpt}, which simulates a software company environment.

Drawing inspiration from these frameworks, we introduce \OURS, a multi-agent collaboration aiming to achieve generalist video generation capabilities similar to those of Sora. \OURS decomposes video generation into subtasks assigned to specialized agents, including prompt enhancement, initial image generation from text, image editing, video creation from images, and video connection. This structured workflow allows for looping and permutation among tasks, facilitating a flexible and comprehensive approach to video generation.

Our system leverages a unique method by starting with both an image and text, simplifying the process as the system primarily needs to predict the progression of the initial image. This approach contrasts with direct text-to-video methods and utilizes SOPs involving human judgment to maintain the diversity, style, and quality of the initial image or video, enhancing editing capabilities.

\begin{figure}[t]
\vspace{-5pt}
\centering
\includegraphics[width=1\linewidth]{figures/method0521.pdf}
\caption{Illustration of SOPs to conduct video-related tasks in \OURS.\yihan{Update this figure to emphasize training.} \yixin{Planning might be replaced with word like \textbf{Support Tasks}}}
\label{method}
\vspace{-8pt}
\end{figure} 

\OURS coordinates text-to-image, image-to-image, image-to-video, and video-to-video agents to handle a broad spectrum of video generation tasks, achieving editing flexibility and visual fidelity comparable to Sora. The comparative analysis presented in our results demonstrates \OURS's adaptability and efficiency in addressing diverse video generation challenges.

We evaluated \OURS using standard metrics from the Vbench benchmark~\citep{huang2023vbench} and our own metrics for specific tasks. Our findings indicate that \OURS excels in text-to-video generation, surpassing other open-source models and ranking closely behind Sora. In other video tasks, \OURS also shows competitive performance, underscoring the robustness and capability of our framework.


We summarize our contributions as follows:


\begin{itemize}[nolistsep, leftmargin=*]
\item In this paper, we present \OURS, an innovative meta-programming framework designed to advance multi-agent collaboration. Distinguished by its structured yet adaptable architecture, \OURS employs a system of agents with clearly defined roles and functions. This architecture equips \OURS to significantly enhance the scope and efficacy of generalist video generation tasks.

\item Our findings indicate that the integration of automated multi-agent cooperation, governed by Standard Operating Procedures (SOPs), significantly enhances both the quality of video generation and the robustness and adaptability of the framework. Moreover, we incorporate human-in-the-loop mechanisms, enabling precise control over the video generation process.

\item \OURS excels in executing a variety of video-related tasks, outperforming existing open-source models. This superior performance highlights \OURS's effectiveness and underscores its potential as a versatile and powerful framework tailored for advanced video generation applications.
\end{itemize}


==> sections/intro-v2.tex <==
Generative AI technologies have significantly transformed various industries, with substantial advancements particularly notable in visual AI through image generation models like Midjourney~\citep{midjourney}, Stable Diffusion~\citep{rombach2022high}, and DALL-E 3~\citep{betker2023improving}. These models have demonstrated remarkable capabilities in generating high-quality images from textual descriptions. However, progress in text-to-video generation, especially for videos exceeding 10 seconds, has not kept pace. Recent developments such as Pika~\citep{pika} and Gen-2~\citep{Gen-2} have shown potential but are limited to producing short video clips.

A major breakthrough occurred with OpenAI’s release of Sora in February 2024—a text-to-video model capable of generating minute-long videos that closely align with textual prompts. Sora excels in various video tasks, including editing, extending footage, offering multi-view perspectives, and adhering closely to user instructions~\cite{openai2024sora}. Despite its impressive capabilities, Sora remains a closed-source system, which poses significant barriers to academic research and development. Its black-box nature hinders the community’s ability to study, replicate, and build upon its functionalities, thereby slowing progress in the field. Attempts to reverse-engineer Sora are exploring potential techniques like diffusion transformers and spatial patch strategies~\citep{sohl2015deep,ho2020denoising,bao2023all,peebles2023scalable}, but a large gap still exists due to the intensive computation required to train everything from scratch with a single model.

To address these challenges, we propose \OURS, a novel multi-agent framework that leverages ideas from standardized operating procedures (SOPs) and employs multiple agents using existing open-source modules to replicate the complex functionalities of Sora. While SOPs and multi-agent systems have been utilized in text-based tasks~\cite{hong2023metagpt}, applying them to text-to-video generation presents unique challenges. Naive multi-agent frameworks~\cite{yuan2024mora,xie2024dreamfactory} often fail because agents lack effective collaboration mechanisms, leading to suboptimal performance. Furthermore, existing multi-agent video generation approaches struggle to balance pipeline automation with fine-grained human control. Collecting video data for training is time-consuming and computationally expensive~\cite{chen2024videocrafter2}, and for quality-critical applications, human-in-the-loop control is necessary to ensure that generated videos meet specific standards~\cite{schramowski2023safe}.

To overcome these fundamental limitations, we introduce several techniques to improve both inter-agent and agent-human collaboration in \OURS. First, we develop a multi-agent fine-tuning approach with a novel modulation factor that enhances coordination among agents, allowing them to collaborate effectively to achieve common goals. Second, we incorporate human-in-the-loop control mechanisms, enabling real-time supervision and adjustments during the video generation process. This approach allows for fine-grained control over the output and improves the overall quality of the generated videos. Third, we employ a data-free training strategy by using large models to synthesize training data, reducing reliance on large labeled datasets and enabling efficient model training without extensive data collection efforts. We summarize the overall pipeline and supported tasks in Figure~\ref{method}.

These techniques collectively improve inter-agent and agent-human collaboration, enhance the quality and diversity of the generated videos, and expand the system’s capabilities to match those of Sora. Our comprehensive experiments on six video generation tasks demonstrate that \OURS achieves competitive performance on VBench~\cite{huang2023vbench}, closely approaching Sora and outperforming existing open-source methods across various tasks. 

\yixin{Please FILL THIS LATER: Specifically, in task XXX, we achieve XX.XX improvement... and in task YYY, we are competitive compared to Sora... Please fill out the new results here with the detailed metrics score presented. }

\begin{figure}[t] \vspace{-5pt} \centering \includegraphics[width=1\linewidth]{figures/ppl.pdf} \caption{Illustration of SOPs to conduct video-related tasks in \OURS.} \label{method} \vspace{-8pt} \end{figure}

We summarize our main contributions as follows:

\begin{itemize}[nolistsep, leftmargin=*]
\item We introduce \OURS, a novel multi-agent framework that leverages existing open-source modules to replicate the functionalities of Sora in text-to-video generation.

\item We address fundamental challenges in agent collaboration for video generation through three key designs: (1) a self-modulated multi-agent fine-tuning approach with dynamic modulation factor for enhanced coordination, (2) human-in-the-loop control mechanisms enabling real-time adjustments, and (3) a data-free training strategy using large models to synthesize diverse training data. These techniques significantly improve inter-agent cooperation and output quality in multi-agent video generation systems.

\item We demonstrate through extensive experiments that \OURS achieves performance comparable to Sora on standard benchmarks, advancing the field of text-to-video generation and providing an accessible platform for future research.
\end{itemize}

==> sections/intro.tex <==

Generative AI technologies have significantly transformed various industries, with substantial advancements particularly notable in visual AI through image generation models like Midjourney~\citep{midjourney}, Stable Diffusion~\citep{rombach2022high}, and DALL-E 3~\citep{betker2023improving}. These models have demonstrated remarkable capabilities in generating high-quality images from textual descriptions. However, progress in text-to-video generation, especially for videos exceeding 10 seconds, has not kept pace. Recent developments such as Pika~\citep{pika} and Gen-2~\citep{Gen-2} have shown potential but are limited to producing short video clips.

A major breakthrough occurred with OpenAI’s release of Sora in February 2024—a text-to-video model capable of generating minute-long videos that closely align with textual prompts. Sora excels in various video tasks, including editing, extending footage, offering multi-view perspectives, and adhering closely to user instructions~\cite{openai2024sora}. Despite its impressive capabilities, Sora remains a closed-source system, which poses significant barriers to academic research and development. Its black-box nature hinders the community’s ability to study, replicate, and build upon its functionalities, thereby slowing progress in the field. Attempts to reverse-engineer Sora are exploring potential techniques like diffusion transformers and spatial patch strategies~\citep{sohl2015deep,ho2020denoising,bao2023all,peebles2023scalable}, but a large gap still exists due to the intensive computation to train everything from scratch with one single model.


To address these challenges, we propose \OURS, a novel multi-agent framework that leverages ideas from standardized operating procedures (SOPs) and employs multiple agents using existing open-source modules to replicate the complex functionalities of Sora. While SOPs and multi-agent systems have been utilized in text-based tasks \cite{hong2023metagpt}, applying them to text-to-video generation presents unique challenges. Naive multi-agent frameworks \cite{yuan2024mora,xie2024dreamfactory} often fail because agents lack effective collaboration mechanisms, leading to suboptimal performance. \yixin{need to give some refer to literature or some results in this paper}
Furthermore, existing multi-agent video generation fails to achieve a good balance between pipeline automation and fine-grained control from the human side. For example, collecting video data for training is time-consuming and requires significant computational resources \cite{chen2024videocrafter2}. For some quality-critical applications, human-in-the-loop control is necessary to ensure the generated videos meet specific quality standards \cite{schramowski2023safe}.
% we might can run some experiment on this baseline after iclr 
% https://arxiv.org/pdf/2408.11788

% TEMPLATE
% For instance, XXX reported a 15% decrease in video quality metrics when compared to single-agent baselines due to inconsistent outputs from different agents \cite{yuan2024mora}. Similarly, in our preliminary experiments with a simple multi-agent setup, we observed a 20% drop in coherence scores and a 25% increase in temporal inconsistencies compared to single-model approaches. These findings underscore the need for more sophisticated coordination strategies in multi-agent video generation systems.

To overcome this fundamental limitation, we introduce several techniques to improve both the interagent and agent-human collaboration in Mora. First, we develop a multi-agent fine-tuning approach with a novel modulation factor that enhances coordination among agents, allowing them to collaborate effectively to achieve common goals. Second, we incorporate human-in-the-loop control mechanisms, enabling real-time supervision and adjustments during the video generation process. This approach allows for fine-grained control over the output and improves the overall quality of the generated videos. Third, we employ a data-free training strategy by using large models to synthesize training data, reducing reliance on large labeled datasets and enabling efficient model training without extensive data collection efforts. We summarize the overall pipeline and supported tasks in Fig \ref{method}. 

These techniques collectively improve interagent and agent-human collaboration, enhance the quality and diversity of the generated videos, and expand the system’s capabilities to match those of Sora. Our comprehensive experiments on six video generation tasks demonstrate that \OURS achieves competitive performance on both VBench \cite{huang2023vbench} and our SoraBench, closely approaching Sora and outperforming existing open-source methods across various tasks. 
\yixin{Speificallly, in task XXX, we achieve XX.XX improvement... and in task YYY, we are competitive compared to Sora... Please fill out the new results here with the detailed metrics score presented. }

\begin{figure}[t]
\vspace{-5pt}
\centering
\includegraphics[width=1\linewidth]{ICLR 2025 Template/figures/ppl.pdf}
\caption{Illustration of SOPs to conduct video-related tasks in \OURS.\yihan{Update this figure to emphasize training.} }
\label{method}
\vspace{-8pt}
\end{figure} 


In summary, our contributions are threefold:
\begin{itemize}[nolistsep, leftmargin=*]
\item We introduce \OURS, a novel multi-agent framework that leverages existing open-source modules to replicate the functionalities of Sora in text-to-video generation.

\item We address the fundamental challenge of agent collaboration by proposing new techniques, including multi-agent fine-tuning with a novel modulation factor, human-in-the-loop control mechanisms, and a data-free training approach using large models to synthesize training data.

\item We demonstrate through extensive experiments that \OURS achieves performance comparable to Sora on standard benchmarks, advancing the field of text-to-video generation and providing an accessible platform for future research.
\end{itemize}


==> sections/method.tex <==
\section{\OURS: A Multi-Agent Framework for Video Generation}
Current text-to-video generation models directly generate videos from textual inputs, which prevents users from supervising key aspects of video quality, style, and other important elements in real time. Inspired by this limitation, we propose a detailed architecture and messaging format specifically designed for each role within the system. As illustrated in Figure~\ref{}, our method employs structured communication among multiple agents and incorporates human interaction at critical points, ensuring step-by-step control over the video generation process, thus improving the overall quality of the final result. Moreover, for each agent, the quality of open-source data has reached its limit in terms of enhancing the final output quality. To further improve video generation quality and control, we designed a data-free, multi-agent self-coordination scheme. This approach enables efficient self-training of models while establishing balanced relationships between agents, further enhancing the controllability and quality of the overall system.

\subsection{Step-controllable Interaction Video Generation with Agents}
\noindent\textbf{Definition and Specialization of Agents. }
The definition of agents enables flexibility in the breakdown of complex work into smaller and more specific tasks, as depicted in Figure \ref{method}. Solving different video generation tasks often requires the collaboration of agents with diverse abilities, each contributing specialized outputs. In our framework, we have 5 basic roles: prompt selection and generation agent, text-to-image generation agent, image-to-image generation agent, image-to-video generation agent, and video-to-video agent. Brief descriptions are below, and detailed definitions can be found in the Appendix.

\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]

\item Prompt Selection and Generation Agent: This agent employs large language models like GPT-4 and Llama~\citep{achiam2023gpt,touvron2023llama} to analyze and enhance textual prompts, extracting key information and actions to optimize image relevance and quality.
\item Text-to-Image Generation Agent: Utilizing models such as those by Rombach~\citep{rombach2022highresolution} and Podell~\citep{podell2023sdxl}, this agent translates enriched textual descriptions into high-quality images by deeply understanding and visualizing complex inputs.
\item Image-to-Image Generation Agent: Referencing Brooks~\citep{brooks2023instructpix2pix}, this agent modifies source images based on detailed textual instructions, accurately interpreting and applying these to make visual alterations ranging from subtle to transformative.
\item Image-to-Video Generation Agent: As described by Blattmann~\citep{blattmann2023stable}, this model transitions static images into dynamic video sequences by analyzing content and style, ensuring temporal stability and visual consistency.
\item Video Connection Agent: This agent creates seamless transition videos from two input videos by leveraging keyframes and identifying common elements and styles, ensuring coherent and visually appealing outputs.
\end{itemize}


\noindent\textbf{Interaction among Agents and Humans. }
The overall process is depicted in Figure~\ref{method}. Specifically, the user inputs a text prompt, which is then modified by the Prompt Enhancement Agent first to a form more suitable for generation. Next, the modified prompt is passed to the Text-to-Image Agent to generate the first frame of the video. At this point, the user has the opportunity to review and confirm whether the tone or quality of the generated first frame meets their expectations. If it does not, the user can request a re-generation or pass it to the Image-to-Image Agent for adjustments. Once the desired first frame is obtained, it is then passed to the Image-to-Video Agent to produce a high-quality video that meets the user's requirements. This step-by-step, independently controllable, and human interactive information transfer method ensures that the final generated video aligns more closely with the user's expectations and achieves higher quality.

Moreover, this procedural design means that the generation process does not have to start from scratch. It enables our framework to handle various tasks, such as image-to-video generation, and even video extension and stitching. For a more detailed list of supported tasks, please refer to the Appendix.


\subsection{Data-free Multi-agent Self-coordinated Training}
\noindent\textbf{LLMs Selection With Human in the Loop. }
Despite the availability of numerous open-source video datasets, their quality varies significantly, making it challenging for the pretrained agents we use to effectively leverage these datasets to improve video generation performance. The issues with existing datasets include high levels of noise, inconsistent content, and a lack of relevance to generation tasks. Manually filtering high-quality data is time-consuming and inefficient, and the most likely outcome is that no new, better data will be found. To address this issue, we introduce the concept of data-free training. This approach involves automatically generating video data and then using a collaborative filtering process between multimodal large language models (LLMs) and human reviewers to ensure the quality and consistency of the training data.

First, we use GPT-4 to generate a large number of text prompts, each of which is used to generate a set of videos. During the filtering process, we employ multimodal large language models that support multi-frame and multi-video inputs to evaluate the generated videos. When multiple LLMs agree on the best video from a set, we directly include it in the training dataset. However, when the LLMs' evaluations differ, we introduce human reviewers for secondary screening.

In such cases, human reviewers evaluate four videos and select the one with the highest quality for inclusion in the training set. If the reviewers determine that none of the four videos meet the quality standard, the entire set is discarded. This approach enhances the stability and robustness of the filtering process by combining LLMs' automated assessments with human judgment, ensuring the model can handle complex or ambiguous cases.

This collaborative filtering strategy between LLMs and human reviewers efficiently filters out low-quality data, avoiding the randomness of a single evaluation method while ensuring the diversity and consistency of the data. This not only improves the efficiency of the data screening process but also enhances the model's ability to handle complex data, ultimately improving training outcomes.


\noindent\textbf{Self-modulated End-to-end Training among Multi-agent. }
The initial design of each agent did not account for the downward transmission of information, which could lead to inefficiencies or errors in communication between agents. Additionally, the impact of each agent on the final result is not uniform. To address these issues, we adopt an end-to-end training approach. Furthermore, we introduce modulation factors to enable efficient coordination and influence distribution between agents, thereby improving the quality of video generation.

Specifically, in the Text-to-Image Agent and Image-to-Video Agent, in addition to the input training data, we also pass a modulation factor, denoted as $z$. The modulation factor $z$ is transmitted between agents, carrying the state information of the preceding agent. Each agent can adjust its output based on the received $z$, for instance, by modifying the style, level of detail, and other attributes of the generated content. During training, the subsequent agent is also capable of transmitting relevant gradient information back to the preceding agent. This design ensures that each agent can dynamically adjust its output according to the state of the preceding agent, enhancing the overall coherence and quality of the generated video.

Let the complete training video be denoted as $x$, composed of frames $x_0, \dots, x_t$. Define $x_{\text{rest}} = \{x_1, \dots, x_t\}$, and let $y$ represent the corresponding description of the video. The modulation factor $z$ is passed between agents and updated at each step.

\begin{equation}
    \frac{\partial L_{total}}{\partial \theta_1}= \frac{\partial L_{1}}{\partial \theta_1}+\frac{\partial L_{2}}{\partial \hat{x_0}}\frac{\partial \hat{x_0}}{\partial \theta_1}+\frac{\partial L_{2}}{\partial z_1}\frac{\partial z_{1}}{\partial \theta_1} 
    \quad 
    \frac{\partial L_{total}}{\partial \theta_{2}} = \frac{\partial L_{2}}{\partial \theta_2}+\frac{\partial L_{2}}{\partial z_2} \frac{\partial z_{2}}{\partial \theta_2}
\end{equation}

Where $\theta$ is the weight of the agents, $L_i$ is the loss of agents, and $z_i$ is the output modulation factor of agents. For the gradient of the initial modulation factor z:

\begin{equation}
    \frac{\partial L_{total}}{\partial z}= \frac{\partial L_{1}}{\partial z}+(\frac{\partial L_{2}}{\partial \hat{x_0}}\frac{\partial \hat{x_0}}{\partial z}+\frac{\partial L_{2}}{\partial z_1}\frac{\partial z_{1}}{\partial z})
\end{equation}

Therefore, during the training process, we update both the model parameters and the modulation factors:
\begin{equation}
    \theta _i\leftarrow \theta _i-\eta_{\theta _i} \frac{\partial L_{total}}{\partial \theta _i} \quad z\leftarrow z-\eta_z\frac{\partial L_{total}}{\partial z} 
\end{equation}

Additionally, an excessively large range of values for the modulation factor may lead to model overfitting or instability during training, while too small a range may limit the model's expressive capacity, preventing it from adequately learning complex patterns in the data. To mitigate the impact of these values on model stability, we use the Sigmoid function for adjustment. The modulation factor is transmitted and modified between agents, enabling information sharing and behavioral regulation. Moreover, restricting the range of the modulation factor ensures the model’s generalization capability. Combined with high-quality training data, this leads to a significant improvement in the quality of the final generated video.






\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/protocol.pdf}
    \caption{A diagram shows the text-to-video generation process in \OURS. \yihan{User input content here can be simpler.} }
    \label{fig:enter-label}
    \vspace{-15pt}
\end{figure}
% Structured communication plays a pivotal role in ensuring the stable operation of multi-agent frameworks. MetaGPT and AutoGen~\citep{hong2023metagpt,wu2023autogen} introduced the concept of using structured communication to coordinate agent interactions in their works. Drawing inspiration from this concept, we propose a detailed schema and message format that is specifically tailored for each role within our system as shown in Figure \ref{fig:enter-label}. This design is particularly focused on the generation and handling of image and video outputs. Our agents are configured to produce dual outputs—textual and media data—which are embedded within messages that encapsulate all essential information. This approach mitigates the risks associated with irrelevant or omitted content, thereby enhancing the efficiency and reliability of the communication process.

% \subsection{LLMs Selection with Human in the Loop}



% \subsection{Iterative Programming with Human in the Loop}
% \label{sec3.3}
% Human oversight and iterative refinement are essential in content generation tasks, improving the quality and precision of the final outputs. Integrating human collaboration within video generation frameworks is pivotal for ensuring that the resulting videos conform to the expected standards.

% As illustrated in Figure \ref{method}, \OURS is engineered to generate videos based on input prompts while executing SOPs under continuous human supervision. This supervisory role enables users to rigorously monitor the process and verify that the outputs align with their expectations. Following each stage, users have the discretion to either advance to the subsequent phase or request a repetition of the previous one, with a maximum of three iterations allowed per stage. This iterative mechanism persists until the output is deemed satisfactory, ensuring high fidelity to user requirements.

==> sections/new_method.tex <==
\section{\OURS: A Multi-Agent Framework for Video Generation}
Current text-to-video generation models directly generate videos from textual inputs, which prevents users from supervising key aspects of video quality, style, and other important elements in real-time. To address this limitation, we propose a novel multi-agent system coupled with a self-modulated training algorithm specifically designed for the video generation task. In the subsequent sections, we outline our approach in detail. In Section~\ref{sec:method:problem}, we formulate the problem definition. Section~\ref{sec:method:arch} describes the design of our multi-agent system and the architecture of our model. Finally, in Section~\ref{sec:method:finetune}, we present our data-free multi-agent fine-tuning method.

\subsection{Problem Definition}
\label{sec:method:problem}
Let $P$ denote a textual prompt describing the desired video content. A video $V$ can be represented as a sequence of frames $V=\{F_1, F_2, \cdots, F_k\}$, where each frame corresponds to an image. The goal is to generate extended-length videos that are semantically consistent with the textual prompt and exhibit high visual quality and temporal coherence. Generally, this problem can be formulated as:
$$
V=G(P)
$$
Where $G$ refers to the generative model that maps a textual prompt input $P$ to a video $V$.
\yihan{Updates denotation here.}

\subsection{\OURS Architecture}
\label{sec:method:arch}
% \yihan{Or sth like Multi-Agent Framework Architecture, will focus more on prompting and connecting the APIs in this section.}
In this section, we introduce our multi-agent video generation system. To address the complexity of generating high-quality, long-duration videos, we propose a multi-agent framework where the generative model $G$ is composed of $n$ collaborating agents $\{A_1, A_2, \cdots, A_n\}$. As shown in Figure~\ref{method}, each agent specializes in a specific subtask and collaborates together within the video generation pipeline. We further introduce the definition of each agent below.

\paragraph{Definition and Specialization of Agents.}
% \yihan{This section will describe the function of each agent.}
The specialization of agents enables flexibility in the breakdown of complex work into smaller and more focused tasks, as depicted in Figure~\ref{method}. In our framework, we have five agents: prompt selection and generation agent $A_1$, text-to-image generation agent $A_2$, image-to-image generation agent $A_3$, image-to-video generation agent $A_4$, and video-to-video agent $A_5$. We present brief descriptions below, and detailed definitions can be found in Appendix~\ref{}.

\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]

\item Prompt Selection and Generation Agent ($A_1$): This agent employs large language models like GPT-4 and Llama~\citep{achiam2023gpt,touvron2023llama} to analyze and enhance textual prompts, extracting key information and actions to optimize image relevance and quality.

% \yihan{Update this description if $A_1$ is trained instead of using APIs.} \zhengqing{$A_1$ dont need to train.}

\item Text-to-Image Generation Agent ($A_2$): Utilizing models such as those by~\cite{rombach2022highresolution} and~\cite{podell2023sdxl}, this agent translates enriched textual descriptions into high-quality images by deeply understanding and visualizing complex inputs.

\item Image-to-Image Generation Agent ($A_3$): Referencing \cite{brooks2023instructpix2pix}, this agent modifies source images based on detailed textual instructions, accurately interpreting and applying these to make visual alterations ranging from subtle to transformative.

\item Image-to-Video Generation Agent ($A_4$): As described by~\cite{blattmann2023stable}, this model transitions static images into dynamic video sequences by analyzing content and style, ensuring temporal stability and visual consistency.

\item Video Connection Agent ($A_5$): This agent creates seamless transition videos from two input videos by leveraging keyframes and identifying common elements and styles, ensuring coherent and visually appealing outputs.
\end{itemize}

\paragraph{General Structure.}
% \yihan{This section will describe the specific model structure.}
\OURS model structure is depicted in Figure~\ref{method}. Specifically, given a user input $T$, the Prompt Enhancement Agent ($A_1$) first refines $T$ into a form better suited for video generation. The enhanced prompt is then passed to the Text-to-Image Agent ($A_2$) to generate the first frame of the video. At this stage, the user can review and confirm whether the tone and quality of the frame meet their expectations. If not, the user can either request a re-generation or pass the frame to the Image-to-Image Agent ($A_3$) for adjustments. Once the desired first frame is finalized, it is forwarded to the Image-to-Video Agent ($A_4$) to generate a high-quality video that aligns with the user's requirements. This step-by-step, independently controllable, and interactive process ensures that the final video more closely meets the user's expectations while maintaining high quality. In cases where a user wishes to generate a continuous video from different video clips, $A_5$ analyzes the final frame of the preceding video and the initial frame of the next and ensures a smooth blending between them.
% \yihan{Add details for $A_5$ video transition agent use cases.}
Moreover, this procedural design means that the generation process does not have to start from scratch. It enables our framework to handle various tasks, such as image-to-video generation, and even video extension and stitching. 
For more details about supported tasks, please refer to Appendix~\ref{}.
In addition to prompt-based generation, \OURS structure also supports task-wise model fine-tuning, ensuring that agents can effectively follow instructions and consistently produce high-quality content.

\subsection{Self-Modulated Multi-Agent Finetuning}
\label{sec:method:finetune}
In this section, we introduce our proposed multi-agent finetuning design, based on the previously described model structure.
% As described in previous sections, our proposed \OURS structure supports multiple tasks by integrating different agents within the general workflow. 
Directly prompting each agent does not account for the downward transmission of information, which could lead to inefficiencies or errors in communication between agents. Additionally, the impact of each agent on the final result is not uniform. To address these issues, we adopt an end-to-end training approach. Our proposed training procedure involves (1) a self-modulation factor to enhance inter-agent coordination, (2) a data-free training strategy to synthesize training data, (3) LLM selection with human-in-the-loop to control the training data quality. In the following sections, we provide a detailed explanation of each component.



% \yixin{I think moderation factor is not appropriate; it actually mean moderation embedding, and the factor actually is the l2 norm of the moderation embedding, distishgush these two concepts are important to make things clear; embedding is vec, factor is scaler. }
\paragraph{Self-modulated Fine-tuning Algorithm.}
\begin{algorithm}[t]
    \caption{Self-Modulated Multi-Agent Fine-tuning}
    \label{alg:self_modulated_training}
    \KwIn{Training data $\mathcal{D} = \{(P^{(i)}_{\text{enh}}, V^{(i)}_{\text{target}})\}_{i=1}^{N}$; batch size $B$; number of epochs $K$; learning rates $\eta_{\theta_i}$, $\eta_{z_i}$; initial model parameters $\theta_i$ for agents $\{A_i\}_{i=0}^{5}$; initial modulation embeddings $\{\mathbf{z}_i = \mathcal{E}_i(\text{"\#900"})\}_{i=1}^{n}$}
    \For{epoch $e = 1$ \KwTo $K$}{
        \ForEach{batch $\{(P^{(b)}_{\text{enh}}, V^{(b)}_{\text{target}})\}_{b=1}^{B}$ in $\mathcal{D}$}{
            Compute text embeddings $\mathbf{e}^{(b)} = \mathcal{E}(P^{(b)}_{\text{enh}})$ for all examples in the batch\;
            \For{$i = 1$ \KwTo $n$}{
                Concatenate agent-specific modulation embedding with text embedding for all examples:
                $\tilde{\mathbf{e}}_i^{(b)} = [\mathbf{e}^{(b)}; \mathbf{z}_i]$\;
                Generate outputs for the batch:
                $O_i^{(b)} = \mathcal{M}_i(O_{i-1}^{(b)}, \tilde{\mathbf{e}}_i^{(b)})$, where $O_0^{(b)} = \emptyset$\;
            }
            Compute the final loss for the batch:
            $L_{\text{final}} = \frac{1}{B}\sum_{b=1}^{B} L(O_n^{(b)}, V^{(b)}_{\text{target}})$\;
            
            \For{$i = 1$ \KwTo $n$}{
                Update agent-specific modulation embedding:
                $\mathbf{z}_i \leftarrow \mathbf{z}_i - \eta_{z_i} \frac{\partial L_{\text{final}}}{\partial \mathbf{z}_i}$\;
                Compute modulation factor:
                $||\mathbf{z}_i||_2 = \sqrt{\sum_{k} z_{i,k}^2}$\;
                Compute modulation factor for model $i$:
                $\alpha_i = ||\mathbf{z}_i||_2 / n$\;
                Update model parameters with dynamic learning rate:
                $\theta_i \leftarrow \theta_i - \alpha_i \eta_{\theta_i} \frac{\partial L_{\text{final}}}{\partial \theta_i}$\;
            }
        }
    }
\end{algorithm}
% Previous methods primarily employ direct end-to-end fine-tuning across the entire task procedure, while others may fine-tune individual agents based on specific tasks. However, both approaches can influence model performance: (1) end-to-end fine-tuning may result in improper loss allocation for each agent, and (2) fine-tuning agents individually can lead to misaligned distributions. To address these issues, we propose a self-modulated finetuning algorithm, specifically designed for multi-agent model structure. The overall procedure is presented in Algorithm~\ref{alg:multi_agent_training}. 
% Specifically, in each agent $\mathcal{M}_i$, in addition to the input, we also pass in a modulation factor $\mathbf{M}_i$ accordingly. $\mathbf{M}_i$ is transmitted between agents, carrying the state information of the preceding agent. Each agent can adjust its output based on the received $\mathbf{M}_i$. The text encoder here is to ....\yihan{Add details here}. 
% By using this trainable modulation factor, the contribution of each agent in the total loss will be reweighted, and hence ensures that each agent can dynamically adjust its output according to the state of the preceding agent. 
% % For instance, by modifying the style, level of detail, and other attributes of the generated content. 
% % During training, the subsequent agent is also capable of transmitting relevant gradient information back to the preceding agent. This design ensures that each agent can dynamically adjust its output according to the state of the preceding agent, enhancing the overall coherence and quality of the generated video.

% \yixin{PLEASE CHECK MY REWRITING:
% }
% To address the limitations of existing fine-tuning approaches, we propose a self-modulated fine-tuning algorithm specifically designed for our multi-agent model structure. This method aims to enhance coordination among agents and improve overall system performance by introducing a modulation embedding that dynamically adjusts the influence of each agent during the generation process. The key motivations behind our approach are to balance the impact of each agent on the final output, improve inter-agent communication and coordination, and allow for dynamic adjustment of agent contributions based on the current task and intermediate outputs.

% Our design introduces a modulation embedding that is concatenated with the text embedding of the enhanced prompt, allowing for fine-grained control over the generation process. This embedding is optimized alongside the model parameters during training, enabling the system to learn optimal coordination strategies. By doing so, we ensure that each agent can adapt its output based on the state of the preceding agent, leading to more coherent and high-quality video generation.

% The implementation of our self-modulated fine-tuning algorithm begins with the initialization of a modulation embedding $\{\mathbf{z}_i\}$ using the text embedding of a special token: $\{\mathbf{z}_i = \mathcal{E}_i(\text{"\#900"})\}$, where $\mathcal{E}_i$ is the text encoder of agent $i$. For each enhanced prompt $P_{\text{enh}}$, we compute its text embedding $\{\mathbf{e}_i = \mathcal{E}_i(P_{\text{enh}})\}$ and concatenate it with the modulation embedding: $\{\tilde{\mathbf{e}}_i = [\mathbf{e}_i; \mathbf{z}_i]\}$. This combined embedding serves as input to the agents.

% Each agent $\mathcal{M}_i$ in the system processes its input and produces an output $O_i$. For the first agent, $O_1 = \mathcal{M}_1(\tilde{\mathbf{e}})$, and for subsequent agents ($i > 1$), $O_i = \mathcal{M}_i(O_{i-1}, \tilde{\mathbf{e}})$. The modulation factor, which influences the impact of each agent, is calculated as the L2 norm of $\mathbf{z}$: $||\mathbf{z}||_2 = \sqrt{\sum_k z_k^2}$.

% During training, we minimize the total loss $L_{\text{total}} = L(O_n, V_{\text{target}})$ between the final output $O_n$ and the target video $V_{\text{target}}$. Both the model parameters $\theta_i$ of each agent and the modulation embedding $\mathbf{z}$ are updated using gradient descent: $\theta_i \leftarrow \theta_i - \eta_{\theta_i} \frac{\partial L_{\text{total}}}{\partial \theta_i}$ and $\mathbf{z} \leftarrow \mathbf{z} - \eta_z \frac{\partial L_{\text{total}}}{\partial \mathbf{z}}$. By optimizing $\mathbf{z}$, the modulation embedding learns to adjust its influence to minimize the loss, effectively enhancing inter-agent coordination and ensuring that each agent can dynamically adjust its output according to the state of the preceding agent.

% The complete training process, including the initialization of the modulation embedding, the forward pass through the agents, and the optimization of both model parameters and the modulation embedding, is detailed in Algorithm~\ref{alg:self_modulated_training}. This algorithm encapsulates our self-modulated fine-tuning approach, providing a comprehensive framework for improving the performance and coordination of our multi-agent video generation system.
Previous methods primarily employ direct end-to-end fine-tuning across the entire task procedure, while others may fine-tune individual agents based on specific tasks. However, both approaches can influence model performance: (1) end-to-end fine-tuning may result in improper loss allocation for each agent, and (2) fine-tuning agents individually can lead to misaligned distributions. To address the limitations of existing fine-tuning approaches, we propose a self-modulated fine-tuning algorithm specifically designed for our multi-agent model structure. This method aims to enhance coordination among agents and improve overall system performance by introducing a modulation embedding that dynamically adjusts the influence of each agent during the generation process. The key motivations behind our approach are to balance the impact of each agent on the final output, improve inter-agent communication and coordination, and allow for dynamic adjustment of agent contributions based on the current task and intermediate outputs.

Our design introduces a modulation embedding that is concatenated with the text embedding of the enhanced prompt, allowing for fine-grained control over the generation process. This embedding is optimized alongside the model parameters during training, enabling the system to learn optimal coordination strategies. By doing so, we ensure that each agent can adapt its output based on the state of the preceding agent, leading to more coherent and high-quality video generation.

The implementation of our self-modulated fine-tuning algorithm begins with the initialization of a modulation embedding $\{\mathbf{z}_i\}$ using the text embedding of a special token: $\{\mathbf{z}_i = \mathcal{E}_i(\text{"\#900"})\}$, where $\mathcal{E}_i$ is the text encoder of agent $i$. For each enhanced prompt $P_{\text{enh}}$, we compute its text embedding $\{\mathbf{e}_i = \mathcal{E}_i(P_{\text{enh}})\}$ and concatenate it with the modulation embedding: $\{\tilde{\mathbf{e}}_i = [\mathbf{e}_i; \mathbf{z}_i]\}$. This combined embedding serves as input to the agents.

Each agent $\mathcal{M}_i$ in the system processes its input and produces an output $O_i$. For the first agent, $O_1 = \mathcal{M}_1(\tilde{\mathbf{e}})$, and for subsequent agents ($i > 1$), $O_i = \mathcal{M}_i(O_{i-1}, \tilde{\mathbf{e}})$. The modulation factor, which influences the impact of each agent, is calculated as the L2 norm of $\mathbf{z}_i $: $||\mathbf{z}_i ||_2 = \sqrt{\sum_k z_k^2}$.

During training, we minimize the total loss $L_{\text{total}} = L(O_n, V_{\text{target}})$ between the final output $O_n$ and the target video $V_{\text{target}}$. Both the model parameters $\theta_i$ of each agent and the modulation embedding $\mathbf{z}_i $ are updated using gradient descent: $\theta_i \leftarrow \theta_i - \eta_{\theta_i} \frac{\partial L_{\text{total}}}{\partial \theta_i}$ and $\mathbf{z}_i \leftarrow \mathbf{z}_i  - \eta_z \frac{\partial L_{\text{total}}}{\partial \mathbf{z}_i }$. By optimizing $\mathbf{z}$, the modulation embedding learns to adjust its influence to minimize the loss, effectively enhancing inter-agent coordination and ensuring that each agent can dynamically adjust its output according to the state of the preceding agent.

The complete training process, including the initialization of the modulation embedding, the forward pass through the agents, and the optimization of both model parameters and the modulation embedding, is detailed in Algorithm~\ref{alg:self_modulated_training}. This algorithm encapsulates our self-modulated fine-tuning approach, providing a comprehensive framework for improving the performance and coordination of our multi-agent video generation system.


% \begin{algorithm}[h]
% \caption{Self-Modulated Multi-Agent Finetuning}\label{alg:multi_agent_training}
% \KwIn{Enhancement prompt $P_{\text{enh}}$, Training video $V_{\text{target}}$, Number of epochs $K$, Text encoders $\mathcal{E}_1, \dots, \mathcal{E}_n$, $n$ models:$\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_n$}
% \KwOut{Updated models: $\mathcal{M}_1, \dots, \mathcal{M}_n$}

% \textbf{Initialization:} \\
% Initialize Modulation Factors: $\mathbf{M}_1 = \dots = \mathbf{M}_n = \texttt{"\#900"}$\;

% \For{epoch $e = 1$ \KwTo $K$}{
%     \For{$i = 1$ \KwTo $n$}{
        
%         $||\mathcal{O}_i|| = \sqrt{\sum_k (\mathcal{E}_i(\mathbf{M}_i)[k])^2}$ \tcp*{Compute the Modulation Factor}

%         Combine $P_{\text{enh}}$ with $\mathbf{M}_i$\;

%         \eIf{$i = 1$}{
%             Generate intermediate output $O_1$ using $\mathcal{M}_1$\;
%         }{
%             Use $O_{i-1}$ as input to $\mathcal{M}_i$ to generate $O_i$\;
%         }
%     }
    
%     $L = \texttt{final}(O_n, V_{\text{target}})$  \tcp*{Compute Final Loss}

%     \For{$i = 1$ \KwTo $n$}{ 
%         $L_i = \frac{||\mathcal{O}_i|| \cdot L}{\sum_{j=1}^{n} ||\mathcal{O}_j||}$ \tcp*{Update $\mathcal{M}_i$ and $\mathbf{M}_i$ parameters using $L_i$}
%     }
% }
% \end{algorithm}

% \begin{algorithm}[H]
%     \caption{Self-Modulated Multi-Agent Fine-tuning =====PLEASE CHECK IT === }
%     \label{alg:self_modulated_training}
%     \KwIn{Training data $\mathcal{D} = \{(P^{(i)}_{\text{enh}}, V^{(i)}_{\text{target}})\}_{i=1}^{N}$; number of epochs $K$; learning rates $\eta_{\theta_i}$, $\eta_z$; initial model parameters $\theta_i$ for agents $\{A_i\}_{i=0}^{5}$; modulation embedding $\mathbf{z} = \mathcal{E}(\text{"\#900"})$}
%     \For{epoch $e = 1$ \KwTo $K$}{
%         \ForEach{training example $(P_{\text{enh}}, V_{\text{target}})$ in $\mathcal{D}$}{
%             Compute text embedding $\mathbf{e} = \mathcal{E}(P_{\text{enh}})$\;
%             Concatenate modulation embedding with text embedding:
%             $\tilde{\mathbf{e}} = [\mathbf{e}; \mathbf{z}]$\;
%             \For{$i = 1$ \KwTo $n$}{
%                 Generate output $O_i = \mathcal{M}_i(O_{i-1}, \tilde{\mathbf{e}})$, where $O_0 = \emptyset$\;
%             }
%             Compute the final loss $L_{\text{final}} = L(O_n, V_{\text{target}})$\;
            
%             Update modulation embedding:
%             $\mathbf{z} \leftarrow \mathbf{z} - \eta_z \frac{\partial L_{\text{total}}}{\partial \mathbf{z}}$\;
%             Compute modulation factor:
%             $||\mathbf{z}||_2 = \sqrt{\sum_{k} z_k^2}$\;
%             \For{$i = 1$ \KwTo $n$}{
%                 Compute modulation factor for model i:
%                 $\alpha_i = ||\mathbf{z}||_2 / n$\;
%                 Update model parameters with dynamic learning rate:
%                 $\theta_i \leftarrow \theta_i - \alpha_i \eta_{\theta_i} \frac{\partial L_{\text{total}}}{\partial \theta_i}$\;
%             }
%         }
%     }
% \end{algorithm}


% \paragraph{Data-free training strategy.}

\begin{algorithm}[t]
    \caption{Data-Free Training Strategy}
    \label{alg:data_free_training}
    \KwIn{Initial agents parameters $\{\theta_i\}$; number of iterations $N$; number of samples per iteration $S$; prompt $P$}
    \KwOut{Trained model parameters $\{\theta_i\}$}
    
    \For{iteration $n = 1$ \KwTo $N$}{
        \For{each prompt $P^{(s)} \in P$}{
            Generate 4 candidate videos $\mathcal{C}_s = \{V_1, V_2, V_3, V_4\}$ using the current agents $\{\theta_i\}$\\;
            Use Multimodal LLM selection with human-in-the-loop control to select the best video $\hat{V}^{(s)}$ from $\mathcal{C}_s$\;
        }
        Construct training dataset for this iteration: $\mathcal{D}_n = \{P^{(s)}, \hat{V}^{(s)}\}_{s=1}^{S}$\;
        Self-Modulated Multi-Agent Fine-tuning using dataset $\mathcal{D}_n$ to update agents parameters $\{\theta_i\}$\;
    }
    \Return{$\{\theta_i\}$}\;
\end{algorithm}

\paragraph{Multimodal LLM selection with human-in-the-loop control.}
Despite the availability of numerous open-source video datasets, their quality varies significantly, making it challenging for the pretrained agents we use to effectively leverage these datasets to improve video generation performance. 
% The issues with existing datasets include high levels of noise, inconsistent content, and a lack of relevance to generation tasks. 
Also, manually filtering high-quality data is time-consuming and inefficient.
% , and the most likely outcome is that no new, better data will be found. 
To address this issue, we introduce a multimodal LLM data selection procedure with human-in-the-loop control. 
% This approach involves automatically generating video data and then using a filtering process between multimodal large language models (LLMs) and human reviewers to ensure the quality and consistency of the training data.
We first sample a batch of candidates from the agent system. 
Based on the generated candidates, we further leverage strong multimodal LLMs that support multi-frame and multi-video inputs to provide evaluation for the candidate set.
When multiple LLMs agree on the best video from a set, we directly include it in the training dataset. However, when the LLMs' evaluations differ, we introduce human reviewers for secondary screening. In such cases, human reviewers evaluate the generated videos and select the one with the highest quality for inclusion in the training set. If the reviewers determine that none of the candidates meet the quality standard, the entire set is discarded. This approach enhances the stability and robustness of the filtering process by combining LLMs' automated assessments with human judgment, ensuring the model can handle complex or ambiguous cases.

\paragraph{Data-free training strategy.}
% During training, rather than directly using open-source datasets, we adopt a data-free strategy to synthesize training data. This approach addresses the varied quality issue of open-source datasets and their lack of intermediate outputs, which are essential for training different agents across various tasks. Given a user input, we first utilize a large language model to generate a diverse set of enhanced prompts. For each prompt, we apply our original workflow—composed of non-finetuned models—to produce data candidates. From this set, we employ the aforementioned selection method to identify high-quality candidates. These selected candidates are then collected and used for end-to-end model finetuning. In a similar manner, the fine-tuned model becomes the starting point for the next round of generation and fine-tuning, enabling iterative improvement.
As detailed in Algorithm~\ref{alg:data_free_training}, during training, instead of using open-source datasets directly, we adopt a data-free strategy to synthesize training data dynamically. This method addresses challenges like inconsistent quality in open-source datasets and the lack of intermediate outputs required for training different agents. Given a user input prompt set \( P = \{ P^{(1)}, P^{(2)}, \dots, P^{(S)} \} \), we first utilize the LLM to generate an enhanced set of diverse prompts \( P_{\text{enh}} = \{ P_{\text{enh}}^{(1)}, P_{\text{enh}}^{(2)}, \dots, P_{\text{enh}}^{(S)} \} \). For each enhanced prompt \( P_{\text{enh}}^{(s)} \), our initial workflow—comprising non-finetuned models with parameters \( \{\theta_i\}_{i=1}^{M} \)—is applied to generate a set of candidate videos \( \mathcal{C}_s = \{ V_1, V_2, V_3, V_4 \} \). Next, we use a human-in-the-loop process, in combination with multimodal LLM selection, to select the highest quality video \( \hat{V}^{(s)} \) from the candidate set \( \mathcal{C}_s \) for each prompt \( P_{\text{enh}}^{(s)} \). The selected video \( \hat{V}^{(s)} \) and corresponding prompt \( P_{\text{enh}}^{(s)} \) form the training dataset for iteration \( n \), denoted by \( \mathcal{D}_n = \{ (P_{\text{enh}}^{(s)}, \hat{V}^{(s)}) \}_{s=1}^{S} \). Using the constructed dataset \( \mathcal{D}_n \), self-modulated multi-agent fine-tuning is performed to update the agent parameters \( \{\theta_i\}_{i=1}^{M} \), where \( M \) is the number of agents involved. The newly fine-tuned model parameters \( \{\theta_i\}_{i=1}^{M} \) then become the starting point for the next round of data generation and fine-tuning, enabling iterative improvement over \( N \) iterations. Thus, after \( N \) iterations, the final optimized agent parameters \( \{\theta_i\} \) are obtained.

